Learning Nonlocal Interactions in Large-Scale Heterogeneous Metamaterials through Scientific Machine Learning

In multiscale systems, nonlocal interactions among spatially distributed constituents can unlock collective, potentially emergent behavior irreducible to individual constituent responses. Beyond characterization, nonlocality in multiscale systems is increasingly viewed as a design element across fracture mechanics, wave physics, and disordered systems. Existing nonlocality theories provide rigorous descriptions and mechanistic insight, but often require prescribed analytic forms, range, symmetries, or periodicity. Machine learning offers a data-driven route to learn interactions, yet principled approaches that tie the network design to physical theory remain nascent. Here we present domain-decomposition attention neural operator (DANO), which learns configuration-dependent interactions in heterogeneous systems governed by linear field equations from field data alone. Through a case study in large-scale optical metasurfaces, we demonstrate DANO's full-field prediction under geometric heterogeneity and across drive conditions, small-to-large domain transfer, and multifunctional inverse design, with learned interactions validated through physics-based interrogation. As an AI-for-Science tool, it supports interaction discovery and scalable, customizable design of nonlocal multiscale systems, including virtual-reality optics.

==> CommPreamble.tex <==
%%% PACKAGES

%\usepackage{amsmath}
%\usepackage{amsthm}
%\usepackage{amssymb}
\usepackage{anyfontsize}
%\usepackage{bm}
\usepackage{enumerate}
\usepackage{esint}
\usepackage{etoolbox}
%\usepackage{fourier}
\usepackage{isomath}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{pgfplots}
\usepackage{scalerel}
\usepackage{stackengine}
\usepackage{tabulary}
\usepackage{tikz}


%%% COMMAND DEFINITIONS

% Formatting Commands

\newcommand{\ds}[1]{\displaystyle{#1}}
\newcommand{\ts}[1]{\textstyle{#1}}

\newcommand{\ns}{\!\!}
\newcommand{\nss}{\ns\ns}
\newcommand{\nsss}{\nss\nss}
\newcommand{\nssss}{\nsss\nsss}

\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\qqqquad}{\qqquad\qqquad}

% General Sets and Spaces

\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\class}[1]{\mathscr{#1}}

% Special Measures
\newcommand{\Leb}{\mathscr{L}}
\newcommand{\Haus}{\mathscr{H}}

% Set Operations

\newcommand{\setm}{\setminus}
\newcommand{\comsub}{\Subset}
\newcommand{\haus}{\mathscr{H}}

% Special Sets

\newcommand{\cmpx}{\mathbb{C}}
\newcommand{\cmpxn}{\cmpx^n}
\newcommand{\cmpxo}{\ov{\cmpx}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\whls}{\mathbb{W}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\rej}{\re^j}
%\newcommand{\rem}{\re^m}
\newcommand{\ren}{\re^n}
\newcommand{\reN}{\re^N}
\newcommand{\renm}{\re^{n\times m}}
\newcommand{\renn}{\re^{n\times n}}
\newcommand{\reNn}{\re^{N\times n}}
\newcommand{\ret}[2]{\re^{#1\otimes #2}}
\newcommand{\ok}{\otimes k}
\newcommand{\reo}{\ov{\re}}

\newcommand{\bll}{\set{B}}
\newcommand{\sph}{\set{S}}
\newcommand{\ann}{\set{A}}
\newcommand{\nhd}{\set{N}}

% Special Spaces

\newcommand{\cnt}{\class{C}}
\newcommand{\bdd}{\class{B}}

% Algebra and Constants

\newcommand{\smfrac}[2]{{\textstyle{\frac{#1}{#2}}}}
\newcommand{\ee}{\mathrm{e}}

% Calculus

\newcommand{\lint}[1]{\int\limits_{#1}}
\newcommand{\luint}[2]{\int\limits_{#1}^{#2}}
\newcommand{\flint}[1]{\fint\limits_{#1}}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\der}[2]{\frac{\dd #1}{\dd #2}}
\newcommand{\derk}[3]{\frac{\dd^{#1} #2}{\dd #3^{#1}}}
\newcommand{\smder}[2]{\smfrac{\dd #1}{\dd #2}}
\newcommand{\smderk}[3]{\smfrac{\dd^{#1} #2}{\dd #3^{#1}}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pderk}[3]{\frac{\partial^{#1} #2}{\partial #3^{#1}}}
\newcommand{\pderkl}[4]{\frac{\partial^{#1} #2}{\partial #3^{#4}}}
\newcommand{\smpder}[2]{\smfrac{\partial #1}{\partial #2}}
\newcommand{\smpderk}[3]{\frac{\partial^{#1} #2}{\partial #2^{#1}}}
\newcommand{\grd}{\te{\nabla}}

% Arc Symbol

\newcommand\widearc[2][\textstyle]{\ensuremath{%
  \!\ns\array[b]{c}\text{\scalebox{2}[1.2]{$#1\frown$}}\\[-1.8ex]#1#2\endarray}\!\ns}

% Vectors

\makeatletter
\newcommand*\bdot{\mathpalette\bdot@{.65}}
\newcommand*\bdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\makeatletter
\newcommand*\bddot{\mathpalette\bddot@{.65}}
\newcommand*\bddot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}
    {$\m@th#1\smash{{}_{\bullet}^{\bullet}}$}}}}}
\makeatother

%\circled[#1]{#2}   % [#1]: size of circle; {#2}: symbol in circle

\newcommand{\circled}[2][]{%
  \tikz[baseline=(char.base)]{%
    \node[shape = circle, draw, inner sep = .5pt]
    (char) {\phantom{\ifblank{#1}{#2}{#1}}};%
    \node at (char.center) {\makebox[0pt][c]{#2}};}}
\robustify{\circled}

\newcommand{\ve}[1]{\vectorsym{#1}}
\newcommand{\valp}{\ve{\alpha}}
\newcommand{\vbet}{\ve{\beta}}
\newcommand{\vvph}{\ve{\vph}}
\newcommand{\vps}{\ve{\psi}}
\newcommand{\vPh}{\ve{\Phi}}
\newcommand{\vxi}{\ve{\xi}}
\newcommand{\vzet}{\ve{\zeta}}
\newcommand{\vom}{\ve{\omega}}
\newcommand{\va}{\ve{a}}
\newcommand{\vf}{\ve{f}}
\newcommand{\vg}{\ve{g}}
\newcommand{\vei}{\ve{i}}
\newcommand{\vK}{\ve{K}}
\newcommand{\vP}{\ve{P}}
\newcommand{\vu}{\ve{u}}
\newcommand{\vv}{\ve{v}}
\newcommand{\vw}{\ve{w}}
\newcommand{\vx}{\ve{x}}
\newcommand{\vy}{\ve{y}}
\newcommand{\vY}{\ve{Y}}
\newcommand{\vz}{\ve{z}}
\newcommand{\vZ}{\ve{Z}}

% Braces

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}
\newcommand{\lc}{\left\{}
\newcommand{\rc}{\right\}}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\lvl}{\left|}
\newcommand{\rvl}{\right|}
\newcommand{\lper}{\left.}
\newcommand{\rper}{\right.}

% Tensors

\newcommand{\te}[1]{\tensorsym{#1}}
\newcommand{\tA}{\te{A}}
\newcommand{\tD}{\te{D}}
\newcommand{\tI}{\te{I}}
\newcommand{\tInn}{\tI^{n\times n}}
\newcommand{\tnu}{\te{\nu}}
\newcommand{\tP}{\te{P}}
\newcommand{\tR}{\te{R}}
\newcommand{\tX}{\te{X}}
\newcommand{\tPhi}{\te{\Phi}}
\newcommand{\tPsi}{\te{\Psi}}

% Matrices

\newcommand{\mx}[1]{\matrixsym{#1}}

% Operators

\def\comp{\operatorname{c}}
\def\bdd{\operatorname{b}}
\def\loc{\operatorname{loc}}
\def\dist{\operatorname{dist}}
\def\diverge{\operatorname{div}}
\def\Hom{\operatorname{Hom}}
\def\sint{\operatorname{int}}
\def\sgn{\operatorname{sgn}}
\def\supp{\operatorname{supp}}
\def\esssup{\operatorname*{ess\;sup}}
\def\essinf{\operatorname*{ess\;inf}}
\def\range{\operatorname{range}}
\def\vspan{\operatorname{span}}
\def\nullsp{\operatorname{Null}}
\def\coker{\operatorname{coker}}
\def\colsp{\operatorname{col}}
\def\rowsp{\operatorname{row}}
\def\range{\operatorname{rng}}
\def\tran{\operatorname{T}}
\def\trace{\operatorname{tr}}
\def\codim{\operatorname{codim}}
\def\rank{\operatorname{rank}}
\def\nullity{\operatorname{nullity}}
\def\DNE{\operatorname{DNE}}
\def\closure{\operatorname{cl}}
\def\interior{\operatorname{int}}
\def\diam{\operatorname{diam}}
\def\conv{\operatorname{Conv}}
\def\card{\operatorname{card}}
\def\proj{\operatorname{proj}}

% Operator Norms

% \opnorm{a}        % normal size
% \opnorm[\big]{a}  % slightly larger
% \opnorm[\Bigg]{a} % largest
% \opnorm*{a}       % \left and \right

\makeatletter
\newcommand{\opnorm}{\@ifstar\@opnorms\@opnorm}
\newcommand{\@opnorms}[1]{%
  \left|\mkern-1.5mu\left|\mkern-1.5mu\left|
   #1
  \right|\mkern-1.5mu\right|\mkern-1.5mu\right|
}
\newcommand{\@opnorm}[2][]{%
  \mathopen{#1|\mkern-1.5mu#1|\mkern-1.5mu#1|}
  #2
  \mathclose{#1|\mkern-1.5mu#1|\mkern-1.5mu#1|}
}
\makeatother

% Other Stuff

\newcommand{\nd}{\quad\text{ and }\quad}
\newcommand{\frl}{\quad\text{ for all }}
\newcommand{\st}{\text{ s.t. }}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\vep}{\varepsilon}
\newcommand{\vph}{\varphi}
\newcommand{\vrh}{\varrho}
\newcommand{\vth}{\vartheta}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wto}{\rightharpoonup}
\newcommand{\supst}[1]{#1^\text{st}}
\newcommand{\supnd}[1]{#1^\text{nd}}
\newcommand{\suprd}[1]{#1^\text{rd}}
\newcommand{\supth}[1]{#1^\text{th}}

\newcommand{\txt}[1]{\textup{#1}}
\newcommand{\gsol}[1]{\underbrace{#1}_{\txt{\small General Solution}}}
\newcommand{\step}[1]{{\textup{Step #1:}}\quad}
\newcommand{\sstep}[1]{{\textup{substep #1:}}\quad}
\newcommand{\rd}{\mathrm{d}}

\newcommand{\dom}{\Omega}
\newcommand{\bnd}{\Gamma}

\newcommand{\bbD}{\mathbb{D}}

\newcommand{\renok}{\ret{n}{k}}


\newcommand{\oA}{\mathscr{A}}
\newcommand{\oD}{\mathscr{D}}
\newcommand{\oL}{\mathscr{L}}
\newcommand{\oP}{\mathscr{P}}
\newcommand{\oR}{\mathscr{R}}
\newcommand{\oT}{\mathscr{T}}

\newcommand{\bi}{\bar{i}}
\newcommand{\ci}{\check{i}}
\newcommand{\hi}{\hat{i}}
\newcommand{\ti}{\tilde{i}}
\newcommand{\hvx}{\hat{\vx}}
\newcommand{\hvy}{\hat{\vy}}
\newcommand{\hS}{\hat{S}}
\newcommand{\whi}{\wh{i}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\whk}{\wh{k}}
\newcommand{\whvx}{\wh{\vx}}
\newcommand{\whvy}{\wh{\vy}}

\newcommand\ochar[1]{\circled[1]{#1}\,}
\newcommand\oempt{\circled[a]{}\,}


\stackMath
\newcommand\reallywidecheck[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}%
}{0.5ex}}%
\stackon[1pt]{#1}{\scalebox{-1}{\tmpbox}}%
}
